On a generalization of the Chvatal-Gomory closure

Many practical integer programming problems involve variables with one or two-sided bounds. Dunkel and Schulz (2012) considered a strengthened version of Chvatal-Gomory (CG) inequalities that use 0-1 bounds on variables, and showed that the set of points in a rational polytope that satisfy all these strengthened inequalities is a polytope. Recently, we generalized this result by considering strengthened CG inequalities that use all variable bounds. In this paper, we generalize further by considering not just variable bounds, but general linear constraints on variables. We show that all points in a rational polyhedron that satisfy such strengthened CG inequalities form a rational polyhedron. We also consider mixed-integer sets defined by linear constraints, to which we extend our polyhedrality result by defining the strengthened CG inequalities on integer variables.

==> 0.abstract.tex <==
\begin{abstract}
Many practical integer programming problems involve variables with one or two-sided bounds. 
Dunkel and Schulz (2012) considered a strengthened version of Chv\'{a}tal-Gomory (CG) inequalities that use 0-1 bounds on variables, and showed that the set of points in a rational polytope that satisfy all these strengthened inequalities is a polytope. 
Recently, we generalized this result by considering strengthened CG inequalities
that use all variable bounds. In this paper, we generalize further by considering not just variable bounds, but general linear constraints on variables. We show that all points in a rational polyhedron that satisfy such strengthened CG inequalities form a rational polyhedron. We also extend this polyhedrality result to mixed-integer sets defined by linear constraints. 
\keywords{Integer programming\and Cutting planes\and Chv\'{a}tal-Gomory cuts\and$S$-free sets\and Chv\'atal-Gomory closure\and Polyhedrality}
\end{abstract}

